Massive Spinor Helicity Amplitudes, Cross Sections, and Coalescence

We examine recent advancements of the spinor helicity formalism of massive particles. Technical aspects about the formulation of massive helicity spinors are presented in detail to analyze the projective-geometry kinematics of helicity spinors as well as the diagrammatical and analytical structure of their interactions. Two new methods for calculating massive cross sections are derived and tested on Bhabha and Compton processes: a quasi-high-energy limit and an assembly of partial cross sections. The acquisition of mass, where ultrarelativistic amplitudes coalesce at low energy, is given a physical interpretation as the localization of particle worldlines in twistor theory. By subsuming the spinor helicity formalism in this way, both spacetime and particle content can emerge from null, lightlike, and timelike twistors.

==> gomezmanuscript.tex <==
% STANDARD PACKAGES
\usepackage{physics}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage[english]{babel} 			% English language hyphenation
\usepackage[parfill]{parskip}    			% Begin paragraphs with empty line
								% \setlength\parindent(or \parskip) after TOC
\usepackage[svgnames]{xcolor} 		% Enabling colors by their 'svgnames'
\usepackage{slashed}				% Feynman slashed notation
\usepackage{dsfont} 					% Math blackboard digits

\usepackage{feynmp}
\newcommand{\marrow}[5]{%
    % Input Arguments: \marrow{name}{arrow_pos}{text_pos}{text}{nodes}
    % name = a, b, c, d, etc
    % arrow_pos = up, down, left, right
    % text_pos = top, bot, lft, rt
    % nodes = {i1,v1}, {i2,v1}
    \fmfcmd{style_def marrow#1
    expr p = drawarrow subpath (1/4, 3/4) of p shifted 6 #2 withpen pencircle scaled 0.4;
    label.#3(btex #4 etex, point 0.5 of p shifted 6 #2);
    enddef;}
    \fmf{marrow#1,tension=0}{#5}
}

\DeclareGraphicsRule{*}{mps}{*}{}
\makeatletter
\def\endfmffile{%
    \fmfcmd{\p@rcent\space the end.^^J%
        end.^^J%
        endinput;
    }%
    \if@fmfio
    \immediate\closeout\@outfmf
    \fi
    \ifnum\pdfshellescape=\@ne
    \immediate\write18{mpost \thefmffile}%
    \fi}
\makeatother

% PAGE MARGINS
\usepackage{geometry} % Required for adjusting page dimensions
\geometry{
	top=2.5cm, % Top margin
	bottom=2.5cm, % Bottom margin
	left=2.5cm, % Left margin
	right=2.5cm, % Right margin
	includehead, % Include space for a header
	includefoot, % Include space for a footer
}

% HEADERS
\usepackage{fancyhdr} 	% Needed to define custom headers/footers
\usepackage{xpatch}	 	% Needed to patch \headrule and make it gold
\pagestyle{fancy}
\fancyhead{} 			% Clear header
\fancyhead[L]{\color{DarkRed}{\sffamily\bfseries\thetitle}}
\fancyhead[R]{\color{DarkRed}{\sffamily\thesubtitle}}
\renewcommand{\headrulewidth}{0.8pt}
\addtolength{\headheight}{0.5pt} % space for the rule
\xpretocmd\headrule{\color{DarkGoldenrod}}{}{\PatchFailed}
\fancyfoot{} 			% Clear footer
\fancyfoot[C]{\color{DarkRed}{\sffamily\bfseries--\:\thepage\:--}}
\fancypagestyle{plain}{% Extra step to apply custom number on first page
	\renewcommand{\headrulewidth}{0pt}
	\fancyhf{}
	\fancyfoot[C]{\color{DarkRed}{\sffamily\bfseries--\:\thepage\:--}}
}

% TITLE
\usepackage{titling} % Allows custom title configuration
\pretitle{
	\vspace{-80pt} % Move the entire title section up
	\fontsize{20}{16}\usefont{OT1}{cmss}{bx}{n}\selectfont
	\color{DarkRed} % Text colour for the title and author(s)
}
\newcommand{\goldrule}{\color{DarkGoldenrod}\rule{\linewidth}{1pt}\\}
\renewcommand{\subtitle}[1]{
\newcommand\thesubtitle{#1}%
\posttitle{
	\par
	\goldrule
	\color{DarkRed}
	\large#1
	\vskip0pt}
}
\preauthor{
	\usefont{OT1}{cmss}{bx}{n}\selectfont
	\color{DarkRed}
	\par
}
\postauthor{}
\predate{
	\usefont{OT1}{cmss}{b}{n}\selectfont
	\color{DarkRed}
	\par
}	
\postdate{
	\vspace{-10pt}
	\par
	\goldrule
}


% ABSTRACT
\renewenvironment{abstract}{
	\usefont{OT1}{cmss}{bx}{n}\selectfont
}


